Risks to Zero Trust in a Federated Mission Partner Environment

Recent cybersecurity events have prompted the federal government to begin investigating strategies to transition to Zero Trust Architectures (ZTA) for federal information systems. Within federated mission networks, ZTA provides measures to minimize the potential for unauthorized release and disclosure of information outside bilateral and multilateral agreements. When federating with mission partners, there are potential risks that may undermine the benefits of Zero Trust. This paper explores risks associated with integrating multiple identity models and proposes two potential avenues to investigate in order to mitigate these risks.

==> Notes.tex <==
The State of the Public Cloud: Security Concerns with Cloud Computing
https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=9249708


==> Sections/COVID19.tex <==
\section{COVID-19}

\sudip{this is too generic, we can cut some words here}
In December of 2019, a handful of pneumonia cases with an unknown etiology in Wuhan, China was brought to the attention of the World Health Organization and within 90 days of that notification, the world was deep in the throes of the COVID-19 pandemic \cite{CDC2022}. In order to protect people from the disease, the world seemingly came to a screeching halt. The response to COVID-19 drove a new model in how personnel operate and communicate which highlighted a need to adopt more modern collaborative technologies. This change, however, brought with it an unprecedented shift in the cybersecurity landscape which acted as a threat surface area multiplier. Further, the impact in various geographical regions not only devastated the economies, but also opened the doors for strategic competitors with strong offensive cyber capabilities to grow their regional footprint. Considering the goal of an enduring capability to facilitate collaboration and sharing with mission partners, it is important to note the changes to the cybersecurity landscape as well as the impact to mission partners.

Almost overnight, the Department of Defense, as with much of the rest of the country, transitioned from a workforce that was predominately in the office to a maximum telework posture. The sudden shift required significant changes in networks to accommodate the number of remote workers. The abrupt change in remote requirements driven by COVID-19 forced a rapid response from agencies in order to provide people the tools they needed to work. \sudip{general stats might not be that useful as this is a very DOD centric article}It is estimated that about 5 percent of the U.S. workforce were remote employees prior to the pandemic; however, the needle moved to approximately 50 percent at the height of telework \cite{Ozimke2021}. According to Lt. Gen Shwedo, that included roughly 4 million DoD personnel \cite{Cohen2020}. This sudden and sustained change to how users connected strained enterprise infrastructures. The United States Air Force (USAF) reported that in the initial weeks, the Virtual Private Network (VPN) capacity which was capped at about 9,000 sessions was upgraded to support 240,000 sessions and the usage jumped 20 fold \cite{Cohen2020}. In addition to increased VPN capacity, the DoD began using commercial applications approved for temporary use. This added a new wrinkle into the daily work life because, as noted that in a DoD IG report, that while most personnel used government issued laptops for remote work, many were using personal devices for their day-to-day unclassified work \cite{IG2021}. The response had effectively introduced the DoD to a new operating model that included access to modern collaborative tools and shed light on the art of the possible \cite{CHES2021}. 


The rapid capability growth brought significant benefit to the end-user in both the ability to operate during the pandemic, and in providing insight into more efficient means of work. However, with these advancements came a drastic increase in complexity and attack surface as cyber professionals needed to consider not only the networks they were charged with protecting, but a myriad of external connections, paths and devices \cite{Erickson2021}. The concerns related to the explosion in access ranges from controlled elements such as VPN to those that are uncontrolled such as a personal device. 

As previously noted, one of the methods of providing access to personnel in a remote environment was to increase the VPN capacity. Notionally, they provide a secure connection into the network by establishing an encrypted tunnel. As with any device, there is a risk of compromise. In October of 2019, the National Security Agency published an advisory on mitigating VPN vulnerabilities identified in major products such as Pulse Secure, Palo Alto GlobalProtect and Fortinet Fortigate \cite{NSA2019}. Additionally, even if an end-user device is an enterprise asset, when operating off the enterprise network it does not have the same network protections. As a result, the benefit of VPN is effectively negated by exposing enterprise routes to potentially compromised devices \cite{Jaffer2021}.

Considering that “99 percent of U.S. government Android users are exposed to hundreds of vulnerabilities due to out-of-date operating systems,” \cite{Lookout2021} it is reasonable to assume that number skyrockets as employees begin to use personal devices which are less likely to benefit from the cyber-hygiene requirements for managed devices. Coupled with a reported 67 percent increase in phishing attacks targeting government credentials, the expansion of mobile device capabilities represents significant growth in an attack vector. When mission partners are taken into account, the risk is significantly greater. Consider only about 9\% of federal employees are using unmanaged devices while 25\% of state and local employees do \cite{Lookout2021}.

The COVID-19 pandemic had overwhelming impacts across the globe; however, some areas felt the impacts more than others. Latin America and the Caribbean, for instance, had reported about 20\% of global cases while only hosting 8\% of the world's population /cite{PostureSOUTHCOM}. In Africa, the U.S. was engaged in assistance efforts in 43 countries and delivered medical supplies valued at approximately \$500M \cite{PostureAFRICOM}. The medical impacts associated with COVID-19 were devastating, but they drove 2nd and 3rd order effects. In Latin America, the per capita income isn’t expected to recover until 2025 which, as of March ’21, was the longest recovery period for any region in the world /cite{PostureSOUTHCOM}. The combination of the medical and economic impacts of COVID-19 around the world has provided opportunity for strategic competitors to offer support as a pretense for advancing their influence in the region. Both USSOUTHCOM and USAFRICOM have noted efforts by the People’s Republic of China (PRC) and Russia to increase their foothold in the regions. Within the USSOUTHCOM’s area of responsibility, the PRC holds \$165B in loans and is using COVID-19 as a pretext to further indebt the region, enhance their integration with the infrastructure and technology. For example, as part of their COVID-19 response, the PRC was offering to donate Huawei technology \cite{PostureSOUTHCOM}.


==> Sections/Conclusion.tex <==
\section{Conclusions and Future Work}
The COCOMs do not operate in isolation within their AORs.  They rely on teamwork with mission partners operating with varying levels of Information Technology infrastructure. In order to facilitate the collaboration and information sharing while minimizing the cost burden, it becomes necessary to utilize the existing capabilities of all mission partners to the maximum extent possible. The recent push towards ZTA, driven by a surge in cyber-attacks, increases the viability of federated unclassified networks; however, there are still security concerns to be considered.\\

The operating assumption of Zero Trust is the network is compromised and therefore an efficient implementation minimizes the ability of an adversary to move laterally within the network. This is accomplished through a combination of micro-segmentation and a continuous, robust authentication/authorization methodology. Micro-segmentation shifts away from the traditional network perimeter that has been blurred by remote workforces, mobile technology and the IoT and focuses security on the resources while the trust algorithm attempts to remove implicit trust by treating all network traffic the same. In an environment where there is centralized control over the critical assets that comprise the ZTA, this paradigm shift represents a significant leap forward in cybersecurity.\\

In a federated networking model, there is a reliance on the maturity of the IT infrastructure of mission partners, specifically their ICAM solutions. Implemented as part of a ZTA, the overall cybersecurity posture is stronger than a perimeter-based model; however, federating still introduces significant risks to the environment. The most obvious risk is associated with capability gaps in providing commensurate levels of context around the requestor side of an access request. The reduced situational awareness increases the likelihood of access with compromised credentials or a compromised device. Beyond context, there are risks associated with supply chain.  The investments by strategic competitors in the way of IT infrastructure introduces opportunities for them to introduce intentionally introduce and exploit vulnerabilities that provide them insight to and control over mission partner ICAM models which would allow access to information shared with the mission partner.\\

ZT represents a significant improvement in the cybersecurity posture of a federated mission system; however, given the vulnerabilities presented, it may be beneficial to consider additional enhancements to assist in minimizing the impacts. Two potential enhancements are the integration of an adaptive neuro-fuzzy inference system (ANFIS) and blockchain. 
\subsection{AFNIS}
The variability of the mission sets the COCOMs collaborate on introduce the need to engage different user architypes. ANFIS is a machine learning model that has been leveraged in behavior analysis. A 2017 experiment using ANFIS for implicit authentication on mobile devices demonstrated a 5\% increase in user recognition rate as well as comparable performance in identifying both informed and uninformed adversary access \cite{Yao}. When paired with designated user types, ANFIS has the potential to provide the TA with behavioral context that can be used to identify a compromise based on both anomalous behavior within the environment and on the end-user device.
\subsection{Blockchain}


==> Sections/Introduction.tex <==
\section{Introduction}


\sudip{read too much like a bulleted list. }

Charles Darwin stated, “In the long history of humankind (and animal kind, too) those who learned to collaborate and improvise most effectively have prevailed.” This sentiment is echoed by senior leaders across the federal government. The 2018 National Defense Strategy highlights the importance of maintaining relationships with mission partners to maintain a favorable balance of power in each of the geographical regions, as well as to ensure a fair share in responsibilities for defense. Further, it focuses on integration and collaboration with mission partners both US interagency and foreign partners /cite{NDS2018}. In his address to Congress on the posture of United States Southern Command (USSOUTHCOM), Admiral Craig S. Faller highlighted the drive for innovation and the need for “open collaboration” with mission partners /cite{PostureSOUTHCOM}. Similarly, when General Stephen J. Townsend delivered his statement on the posture of United States Africa Command (USAFRICOM), he stated the importance of multi-national, as well as bilateral, cooperation \cite{PostureAFRICOM}.The goal is to achieve synergy by allowing the collaboration to foster improvisation and in turn, innovation. Unfortunately, the personnel within the Department of Defense are far too often forced to improvise in order to collaborate.

The need to collaborate goes beyond the ability to prosecute a war. The Combatant Commands (COCOMs) are regularly engaged in military operations other than war ranging from counter narcotics to humanitarian aid and disaster relief (HA/DR) missions. To that end, COCOMs are in need of an enduring, integrated suite of collaborative tools capable of storing, processing and transmitting unclassified data up to and including Controlled Unclassified Information (CUI) with mission partners across their Areas of Responsibility. However, recent events have highlighted growing gaps relative to this requirement and cybersecurity concerns across the federal government. The Coronavirus Disease 2019 (COVID-19) response both heightened awareness of the need for modern collaboration tools and substantially increased the attack surface of enterprise networks. This triggered both an uptick in cyber attacks and strategic posturing by countries with aggressive state-sponsored cyber actors.

The changing landscape and rapid growth in vulnerabilities forced the federal government to acknowledge the need for a paradigm shift in cybersecurity. To that end, the migration to a Zero Trust Architecture for all Federal Information Systems was directed.  This paper investigates the requirement for a modernized Unclassified Information Sharing Service, the subsequent impact of COVID-19 and the extent to which a migration to Zero Trust mitigates the risks inherent in information sharing and what additional steps may be necessary to deliver a full capability suite. 


\sudip{In this paper, we ...}

UISS



\sudip{Your proposed solution idea?/opinion?}

\sudip{what will be the impact of your proposed solution?}

\sudip{Main Contributions?}

ZTA is all in 

limitations of ZTA that prohibit International mission pratners 

Identity specific concerns 

Threats 



The Department of Defense is making a concerted effort to transition information systems to Zero Trust Architectures (ZTA) to enhance their cybersecurity postures. Zero Trust assumes the network is compromised and focuses on minimizing the potential impact of a cyber-attack by strengthening the algorithm used to authenticate and authorize a session while also reducing the ability to move laterally within the network. The effectiveness of ZTA is largely dependent on access to information specific to each request; however, in a federated network model where participating organizations are responsible for bringing their own Identity, Credential and Access Management (ICAM) model, the amount and fidelity of information available may undermine the benefits of ZTA. 

In  this paper, we investigate the impact of substandard or compromised ICAM models on a federated network implementing ZTA. Given a mission partner with a deficient ICAM solution with whom data is being shared, it is expected that all resources shared with said partner are compromised and raise the potential for proliferation as those resources are access by other mission partners. It is assumed there is a centrally managed environment that effectively implements the micro-segmentation principles of ZTA such that access is restricted to the requested resource during a given session. This assumption allows focuses the review on the impact of the deficient ICAM solution on this federated environment by assessing the effects on the trust algorithm.


==> Sections/UISS.tex <==
\section{Unclassified Information Sharing Service}
This Unclassified Information Sharing Service (UISS) is intended to provide an enduring enterprise solution that enables COCOMs, traditional and “non-traditional” mission partners to share information through the use of integrated commercial-off-the-shelf (COTS) products across various devices\cite{PB2019}. The UISS is an element of the Mission Partner Environment (MPE), the United States’ framework to support the North Atlantic Treaty Organization’s (NATO) Federated Mission Networking (FMN) construct \cite{Sullivan2021}, that focuses on collaboration and sharing with mission partners at the unclassified level, including CUI. To better understand the requirements and risks associated with UISS, the subsequent sections will take a look at types of international mission partners, discuss requirements around protecting CUI and provide some assumptions related to mission partner capabilities.

\subsection{International Mission Partners}
The international mission partners COCOMs work with take on a variety of forms, the most obvious being foreign military. However, there is a significant amount of cooperation that occurs with other agencies. In January 2010, USSOUTHCOM responded to a request for earthquake relief support in Haiti. This HA/DR operation required coordination with multiple international organizations, including foreign government agencies, nongovernment agencies and foreign militaries. In order to effectively share information, data was kept unclassified to the maximum extent possible and public platforms were used for dissemination \cite{arroyoCenter}. Another example of cooperation with international partners can be found in a recent partnering between USAFRICOM, the International Criminal Police Organization (INTERPOL) and local law enforcement from several West African nations. The operation targeted illegal fishing and “other maritime crimes” along the West African coast \cite{maritime}. 

\subsection{Controlled Unclassified Information}  
The category of CUI was defined by Executive Order 13556 as a means of providing a uniform method for agencies in the executive branch to mark unclassified data that requires additional protective measures, such as health information. The DoD adopted CUI as an official marking through the issuance of DoDI 5200.48 which defined a phased approach to implementing the CUI Program, outlined roles and responsibilities, and described general requirements for handling CUI. Of particular interest to the UISS requirement set are section 3.9 which defines release and disclosure \cite{DoDI520048}. 

\subsubsection{Release and Disclosure} 
As noted above, DoDI 5200.48 dedicates section 3.9 to discussing release and disclosure requirements for CUI data. For example, data controlled as NOFORN is not releasable to foreign mission partners; however, it may need to reside in UISS due to a need to release to non-foreign entities such as the Federal Emergency Management Agency. Similarly, data controlled as “CUI//REL To USA, FVEY” is releasable to members of the Five Eyes alliance \cite{CUI_PPT}. A comparable protection requirement exists for mission partner data. The MPE framework is designed to facilitate collaboration and sharing with “participants within a specific partnership or coalition” \cite{CJCSI629001}. The implication is a requirement to ensure data is only shared within designated groups. For example, assume there are existing agreements between the United States, country A and country B, as depicted in \hl{Figure 1}. In this image, the overlapping areas represent shared data based on these partnerships. Each country contributing data to the environment expects the information it uploads to the system to be protected accordingly. That is to say, data transferred to the United States as part of a bilateral agreement with country A must not be released to country B without the express consent of country A.

==> Sections/ZeroTrust.tex <==
\section{Zero Trust} 
In the tenth year of the Trojan War, after siege tactics and brute force had failed, Odysseus devised a strategy that would see the Trojans unwittingly help the Greeks breach the 5m thick and 8m high defensive walls of Troy. Once breached, the Greeks had access to the entire city, and it fell within a matter of days \cite{Struck2020}. More than 3,100 years later, the battlefield may have changed, but when it comes to cyberspace, perimeter-based defense is still the predominant model and attackers are taking advantage of it. Before diving into Zero Trust, a brief listing of some recent notable cyber-attacks will be provided to offer context around how adversaries are taking advantage of the vulnerabilities and areas Zero Trust has the potential to enhance cyber defense.
\subsection{Recent Attacks}
\subsubsection{Marriott}
Within a two-year timeframe, Marriott International, an international hotel chain, suffered from two major data breaches. The first occurred in 2018 when over 500 million customer records were stolen \cite{MI2018}. The second occurred in early 2020 and saw 5 million accounts accessed \cite{MI2020}. There set of information on how the hacks occurred is not complete; however, there is sufficient detail to shed light on certain flaws with a traditional perimeter defense model. 
In 2018, a database query was flagged by a security tool as being suspect. The resulting investigation found that an administrative account had been compromised and a couple of tools used for stealing passwords, including a Remote Access Trojan.
\subsubsection{Solar Winds}
On December 8, 2020, it was discovered that SolarWinds had been compromised. The hack, attributed to Russia, affected approximately 17,000 of SolarWinds clients, including several federal agencies such as the Department of Homeland Security and the Department of Defense. This is a prime example of a supply chain attack. The attackers targeted a third-party vendor, Orion, that had a long-standing relationship with SolarWinds. By infiltrating Orion, when clients of SolarWinds updated their software, they inadvertently loaded malware onto the devices giving hackers access to their networks, which in many instances resulted in significant data breaches /cite{SolarWinds}.
\subsubsection{Colonial Pipeline}
In May of 2021, the Colonial Pipeline was shut down due to a ransomware attack. While the attack impacted the business systems, the pipeline was shut down for 7 days as a precaution. As with the SolarWinds attack, this was attributed to Russian hackers. In this case, the Russian-based group DarkSide claimed responsibility /cite{cyberattacksICS}. 
The hackers gained access to Colonial Pipeline’s system using compromised credentials. Utilizing those credentials, they were able to access the system through an inactive Virtual Private Network account that did not support multi-factor authentication. DarkSide was able to exfil 100GB of data and encrypt several corporate systems such as billing. This allowed DarkSide to ransom both the data and the ability to decrypt the systems /cite{ICStrends}. The hack of the Colonial Pipeline was the proverbial straw that broke the camel's back and within a few days Executive Order 14028 was signed.

\subsection{What is Zero Trust}
On May 12, 2021, Joseph R. Biden Jr., President of the United States, signed into effect Executive Order 14028: Improving the Nation’s Cybersecurity. Prompted by recent “sophisticated and malicious” \cite{Biden} cyber-attacks, the order acts as a catalyst for federal agencies to take necessary and immediate steps to coordinate with industry on improving information sharing, adopting best practices and, among other things, migrating Federal Information Systems from perimeter-based security to a Zero Trust Architecture (ZTA).   
In order to understand the potential impact of Zero Trust on UISS, the next sections will discuss some of the recent, notable cyber-attacks, the tenets of Zero Trust and the pros and cons associated with it. \\
The preceding section on cyberattacks showed common themes related to perimeter-based cybersecurity concerns, namely trust and lateral movement. While a ZTA doesn’t eliminate these risks, it takes steps to minimize the likelihood and reduce the potential impact. As the name implies, the foundation of Zero Trust is removing, to the maximum extent possible, trust from cybersecurity architectures. That effectively means users, networks and devices no longer receive the inherent trust built into a perimeter-based model because all traffic is considered untrusted \cite{Forester}. 
\\

One of the major underpinnings of a ZTA is the deperimeterization of the enterprise network. While in the context of ZTA, deperimeterization is discussed in terms of micro-segmentation, the concept dates back to a 2001 research paper by Jon Measham and became a core element of the Jericho Forum which advanced the concept over the next decade \cite{chieftech}.  In establishing a vision for deperimeterization, one of the areas the Jericho Forum focused on was the establishment of trust models including dynamic and transitive trust ideas. Then in 2010, John Kindervag advanced the concept of deperimeterization by introducing ZTA which removed trust from the equation, sort of. Zero Trust and deperimeterization do not remove trust and perimeters from the enterprise networks. They focus on taking the “arbitrary” out of networking.  Today, more than ever, the traditional boundaries have been obfuscated by advancements in mobile technology, adoption of cloud computing and the Internet of Things. ZTA strives for a paradigm shift away from the traditional model of being more concerned with “roads than with destinations” \cite{Forrester}. With respect to trust, consider the adage “trust but verify.” Removing the arbitrary trusts out of the verify process shifts the model to putting all traffic through the same rigorous assessment process and continually reevaluating approvals.

\subsection{NIST SP 800-207}

The National Institute of Standards and Technology (NIST) published Special Publication 800-207 in August ’20. The intent of the document is to standardize the terms and definitions around ZTA, as well as define potential implementation strategies in order to assist federal information system owners in migrating to a ZTA. It provides a framework for agencies to begin assessing the options related to ZTA and the level of effort to begin transitioning. Rather than summarize the entirety of NIST SP 800-207, this section will focus on section three of the document which defines the components of ZTA.
\\\\
There are two primary components in ZTA, the Policy Decision Point (PDP) and the Policy Enforcement Point (PEP). The names are rather self-explanatory.   The PDP assess the request for access, while the PEP manages the access request by implementing the PDP’s decision and monitoring the connection in support of a continuous feedback loop with the PDP. \\

\subsubsection{Trust Zone}

As mentioned earlier, ZTA does not eliminate trust. The micro-segmentation of the network serves to reduce the “implicit trust zone.” This trust zone includes everything inside a given segment protected by the PDP/PEP.  Therefore, within a trust zone, lateral movement is possible. However, the smaller the segment, the smaller the threat surface. The document draws a parallel to passing through the security checkpoint at an airport with the boarding area being the trust zone. Once through security, passengers can access resources within the zone and move laterally between gates, restaurants, and shops.\\

\subsubsection{Trust Algorithm}

The Trust Algorithm (TA) is the heart of ZTA because it is the assessment process used by the PDP to determine whether to grant access to a resource. Access to critical data feeds is critical in ensuring the TA is capable of making informed decisions. Aside from information relative to the credentials and rights of the requestor, the TA should require information relative to the security posture of both the requesting device and the requested resource and threat intelligence.  There are a couple of variants of the TA, which are not mutually exclusive, defined.  Relevant to the data feeds is “singular versus contextual” which accounts for whether the TA has access to the history of requests. Ideally, a contextual TA will be used given it provides insight into the user behavior and can help ensure that use meets behavioral norms. The second variant is “criteria- versus score-based.” 


\sudip{Limitations of Zero trust in UISS}


